Maximum energy achievable in supernova remnants: self-consistent simulations

It has been long believed that oblique and quasi-perpendicular configurations in supernova remnants (SNRs) were inefficient at injecting ions into diffusive shock acceleration (DSA), and that the highest energy Galactic cosmic rays (CRs) must come from parallel or quasi-parallel shocks. However, recent 3D kinetic simulations have shown that high-obliquity shocks can successfully energize particles and produce amplified magnetic fields in the upstream. We aim to investigate the maximum energy particles it is possible to produce in oblique and quasi-perpendicular shocks and whether they are capable of triggering the non-resonant hybrid instability (NRHI). We present a novel setup for hybrid simulations of non-relativistic shocks that use a "faux shock" boundary condition instead of a real shock to significantly reduce the computational cost and that can be run for long enough to study the late-time behaviors of these systems. Our results show that it may be possible for oblique and quasi-perpendicular shocks to transition from early periods of shock drift acceleration (SDA) into DSA at later times, giving particles a brief period of rapid acceleration followed by a long-duration, self-sustaining period of slower energy growth. Furthermore, we find evidence that the NRHI is triggered in the upstream at late times. Oblique and quasi-perpendicular shocks may be an important contributor to high energy CRs, potentially even responsible for the knee in the CR energy spectrum.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

